Longitudinal Position and Cancer Risk in the United States Revisited

Background: The debate over daylight saving time has surged, with interests in the effects of sunlight exposure on health. \commentnj{Prior studies simulated daylight saving time and standard time conditions by analyzing different locations within time zones and neighboring areas across time zone borders. Methods: We analyzed cancer incidence rates from various longitudinal positions within time zones and at time zone borders in the contiguous United States. Using data from State Cancer Profiles (2016-2020), we analyzed total cancer of 19 types and specific rates for eight cancers, adjusted for age and includes all demographics. Log-linear regression is used to replicate a previous study, and spatial regression models are employed to explore discontinuities at borders. Results: Cancer rate differences lack statistical significance within time zones and near borders for total cancer and most individual cancers. Exceptions included breast, prostate, and liver \& bile duct cancers, which exhibited significant relationships with relative position at the 95\% significance level. Breast and liver and bile duct cancers saw decreases, while prostate cancer incidence increased from west to east within time zones. Conclusions: Relative position does not have a significant impact on cancer incidence, hence cancer development in general. Isolated exceptions may warrant further investigation as more data becomes available. Impact: Our findings challenge prior research, revealing numerous inconsistencies. These disparities urge a reconsideration of the potential disparities in human health associated with daylight saving time and standard time. They offer insights contribute to the ongoing discussion surrounding the retention or abandonment of DST.

==> Notes.tex <==
statistics in medicine?

% Checking to make sure citations are working:  \cite{gu2017longitude}.  Good.

Everything right now is temporary; I put authors alphabetically (roughly) for now so it doesn't output an error message.  Feel free to make any changes that you want!

From jr:  ``We need two things for srdd: p value and something like bootstrap (p value, sensitivity analysis.)''


other articles published by Statistics in Medicine that may be helpful:

\url{https://onlinelibrary.wiley.com/doi/10.1002/sim.9425}

\url{https://onlinelibrary.wiley.com/doi/10.1002/sim.9422}

\url{https://onlinelibrary.wiley.com/doi/10.1002/sim.9384}


5/25
p-value:
test significant diff on the border
ex. linear models and use F-test

sensitivity analysis bootstrap:

% One suggestion for writing:  you should use the ``\textbackslash cite'' function rather than typing out the citation in text and include the bibtex reference in ``ref.bib''.  For example, write \cite{giuntella2019sunset} instead of Giuntella and Mazzonna.  This way, if we want to change citation formats (say from APA to ICM or MLA), then we don't have to go back and reformat the text, but rather just change the bibliography style at the end of the document.

==> cancer_reg_output_BIG.tex <==
% Date and time: Tue, Feb 14, 2023 - 22:12:57
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Breast Cancer - Reported Coefficients of Linear Model by Relative Position 
            (with 95\% Confidence Interval)} 
  \label{linearmod_relpos} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Cancer Incidence Rate} \\ 
\hline \\[-1.8ex] 
 Relative Position & -0.285$ $(-0.469$, $-0.101)^{***} \\ 
  Latitude & 0.514$ $(0.165$, $0.862)^{***} \\ 
  High School & 45.179$ $(20.773$, $69.584)^{***} \\ 
  Some College & 57.917$ $(37.167$, $78.666)^{***} \\ 
  College and Above & 82.081$ $(60.290$, $103.872)^{***} \\ 
  Elevation & -0.006$ $(-0.009$, $-0.003)^{***} \\ 
  Medical Doctor pc & 4.735$ $(-296.566$, $306.035) \\ 
  Median Income & 0.00004$ $(0.00000$, $0.0001)^{**} \\ 
  Obesity Rate & 22.247$ $(8.124$, $36.369)^{***} \\ 
  Smoking Rate & -105.899$ $(-144.468$, $-67.330)^{***} \\ 
  PM2.5 (air pollution) & 0.138$ $(-0.155$, $0.431) \\ 
  Water Violation & 1.408$ $(0.522$, $2.294)^{***} \\ 
  Race (White) & -77.824$ $(-146.452$, $-9.195)^{**} \\ 
  Race (Black) & -66.783$ $(-135.908$, $2.343)^{*} \\ 
  Race (Native) & -105.620$ $(-178.470$, $-32.770)^{***} \\ 
  Race (Asian) & -129.830$ $(-203.036$, $-56.624)^{***} \\ 
  Race (Hispanic) & -89.638$ $(-158.906$, $-20.371)^{**} \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{2,615} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.534} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.523} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.388 (df = 2554)} \\ 
F Statistic & \multicolumn{1}{c}{48.760$^{***}$ (df = 60; 2554)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


% Date and time: Tue, Feb 14, 2023 - 22:21:04
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Prostate cancer - Reported Coefficients of Linear Model by Relative Position 
            (with 95\% Confidence Interval)} 
  \label{linearmod_relpos} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Cancer Incidence Rate} \\ 
\hline \\[-1.8ex] 
 Relative Position & 0.387$ $(0.123$, $0.650)^{***} \\ 
  Latitude & 0.700$ $(0.198$, $1.203)^{***} \\ 
  High School & 37.997$ $(2.708$, $73.286)^{**} \\ 
  Some College & 86.469$ $(56.234$, $116.704)^{***} \\ 
  College and Above & 71.577$ $(39.726$, $103.428)^{***} \\ 
  Elevation & -0.005$ $(-0.009$, $-0.002)^{***} \\ 
  Medical Doctor pc & -322.516$ $(-773.165$, $128.133) \\ 
  Median Income & 0.00004$ $(-0.00001$, $0.0001) \\ 
  Obesity Rate & 15.190$ $(-5.156$, $35.537) \\ 
  Smoking Rate & -104.505$ $(-161.113$, $-47.896)^{***} \\ 
  PM2.5 (air pollution) & 0.107$ $(-0.319$, $0.533) \\ 
  Water Violation & 2.400$ $(1.119$, $3.681)^{***} \\ 
  Race (White) & 209.432$ $(110.637$, $308.228)^{***} \\ 
  Race (Black) & 288.464$ $(188.715$, $388.212)^{***} \\ 
  Race (Native) & 209.595$ $(104.050$, $315.139)^{***} \\ 
  Race (Asian) & 157.325$ $(51.945$, $262.706)^{***} \\ 
  Race (Hispanic) & 219.558$ $(119.763$, $319.353)^{***} \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{2,623} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.573} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.563} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.612 (df = 2562)} \\ 
F Statistic & \multicolumn{1}{c}{57.412$^{***}$ (df = 60; 2562)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


% Date and time: Tue, Feb 14, 2023 - 22:32:26
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Liver Cancer - Reported Coefficients of Linear Model by Relative Position 
            (with 95\% Confidence Interval)} 
  \label{linearmod_relpos} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Cancer Incidence Rate} \\ 
\hline \\[-1.8ex] 
 Relative Position & -0.084$ $(-0.158$, $-0.010)^{**} \\ 
  Latitude & 0.071$ $(-0.067$, $0.208) \\ 
  High School & -5.935$ $(-16.751$, $4.881) \\ 
  Some College & -1.847$ $(-10.838$, $7.145) \\ 
  College and Above & -13.262$ $(-22.371$, $-4.154)^{***} \\ 
  Elevation & -0.001$ $(-0.002$, $-0.0002)^{**} \\ 
  Medical Doctor pc & 430.093$ $(318.346$, $541.841)^{***} \\ 
  Median Income & 0.00000$ $(-0.00001$, $0.00002) \\ 
  Obesity Rate & -4.150$ $(-10.068$, $1.768) \\ 
  Smoking Rate & 39.361$ $(24.681$, $54.041)^{***} \\ 
  PM2.5 (air pollution) & 0.018$ $(-0.092$, $0.127) \\ 
  Water Violation & -0.344$ $(-0.670$, $-0.018)^{**} \\ 
  Race (White) & -51.620$ $(-78.410$, $-24.830)^{***} \\ 
  Race (Black) & -45.369$ $(-72.414$, $-18.324)^{***} \\ 
  Race (Native) & -59.876$ $(-89.073$, $-30.678)^{***} \\ 
  Race (Asian) & -39.608$ $(-68.239$, $-10.976)^{***} \\ 
  Race (Hispanic) & -43.964$ $(-71.080$, $-16.847)^{***} \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{1,117} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.556} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.530} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.404 (df = 1056)} \\ 
F Statistic & \multicolumn{1}{c}{21.996$^{***}$ (df = 60; 1056)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

% Date and time: Tue, Feb 14, 2023 - 22:42:40
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Lung cancer - Reported Coefficients of Linear Model by Relative Position 
            (with 95\% Confidence Interval)} 
  \label{linearmod_relpos} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Cancer Incidence Rate} \\ 
\hline \\[-1.8ex] 
 Relative Position & 0.140$ $(-0.023$, $0.302)^{*} \\ 
  Latitude & -0.025$ $(-0.306$, $0.257) \\ 
  High School & 16.051$ $(-4.794$, $36.895) \\ 
  Some College & 27.186$ $(9.601$, $44.770)^{***} \\ 
  College and Above & -22.630$ $(-40.985$, $-4.274)^{**} \\ 
  Elevation & -0.009$ $(-0.011$, $-0.007)^{***} \\ 
  Medical Doctor pc & 958.870$ $(711.023$, $1,206.717)^{***} \\ 
  Median Income & 0.00001$ $(-0.00002$, $0.00004) \\ 
  Obesity Rate & 30.056$ $(18.115$, $41.998)^{***} \\ 
  Smoking Rate & 226.326$ $(194.047$, $258.606)^{***} \\ 
  PM2.5 (air pollution) & 0.346$ $(0.115$, $0.577)^{***} \\ 
  Water Violation & 0.399$ $(-0.325$, $1.122) \\ 
  Race (White) & -241.304$ $(-298.072$, $-184.536)^{***} \\ 
  Race (Black) & -246.785$ $(-304.098$, $-189.472)^{***} \\ 
  Race (Native) & -311.201$ $(-371.743$, $-250.659)^{***} \\ 
  Race (Asian) & -224.304$ $(-284.614$, $-163.994)^{***} \\ 
  Race (Hispanic) & -259.359$ $(-316.784$, $-201.934)^{***} \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{2,441} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.823} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.818} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.431 (df = 2380)} \\ 
F Statistic & \multicolumn{1}{c}{184.027$^{***}$ (df = 60; 2380)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 
